Open-Source LiDAR Time Synchronization System by Mimicking GNSS-clock

Data fusion algorithms that employ LiDAR measurements, such as Visual-LiDAR, LiDAR-Inertial, or Multiple LiDAR Odometry and simultaneous localization and mapping (SLAM) rely on precise timestamping schemes that grant synchronicity to data from LiDAR and other sensors. Poor synchronization performance, due to incorrect timestamping procedure, may negatively affect the algorithms' state estimation results. To provide highly accurate and precise synchronization between the sensors, we introduce an open-source hardware-software LiDAR to other sensors time synchronization system that exploits a dedicated hardware LiDAR time synchronization interface by providing emulated GNSS-clock to this interface, no physical GNSS-receiver is needed. The emulator is based on a general-purpose microcontroller and, due to concise hardware and software architecture, can be easily modified or extended for synchronization of sets of different sensors such as cameras, inertial measurement units (IMUs), wheel encoders, other LiDARs, etc. In the paper, we provide an example of such a system with synchronized LiDAR and IMU sensors. We conducted an evaluation of the sensors synchronization accuracy and precision, and state 1 microsecond performance. We compared our results with timestamping provided by ROS software and by a LiDAR inner clocking scheme to underline clear advantages over these two baseline methods.

==> _notes.tex <==
\mf{More tech descr}

\mf{accuracy}

\mf{sync to error}

\mf{expand results and methodology?}

The INERTIAL 2022 Organizing Committee

****************************************

Reviewer 1 Comments

****************************************

%First off, the reviewer commends the authors efforts to create open-source software and detailed documentation of the needed hardware so that others may benefit from their work. However, in order to be suitable for acceptance, the reviewer notes that the following areas should be addressed:

\textcolor{green}{DONE} \mf{HW sync details in abstract} -While the abstract format precludes providing exhaustive details of the method used for time synchronization, no details about how hardware time synchronization works is provided. 

\textcolor{green}{DONE} \mf{make source available} The authors do note that this information will be released once accepted, but this introduces issues related to \textbf{assessing the novelty} of the work and potential limitations, for example, due to the underlying model or assumptions used for time synchronization. 

\mf{innovative in comparison to versavis} In regards to novelty, the authors third reference on Versavis is also on an open-source hardware time synchronization method that integrates with ROS. 

The authors need to clarify what is new or innovative. 
During initialization, Versavis triggers using a slow 1 Hz signal. This is very similar to a 1 PPS signal derived from GNSS. 

In regards to modeling and assumptions, this information needs to be provided \textbf{so that potential users can assess if the presented method is suitable} for their application. 

For example, \textbf{does this approach allow for sensors to be triggered and sampled independently or does the hardware enforce uniform triggering and sampling?}

\mf{provide accuracy} -The authors report an impressive time synchronization precision. 

However, given that sampling offsets between the IMU and LIDAR can introduce issues with SLAM, shouldn’t \textbf{accuracy} of time synchronization should also be assessed? 

If the authors can show that accuracy is not significant for their selected application of SLAM and that a biased but very precise time synchronization can be used, this would be an important result.

However, if accuracy is more important, this information should be reported.

\mf{Show example of sync to position error} -The authors note that time synchronization errors become a more significant issue during high dynamic conditions. 

To provide context to conference attendees that are not familiar with robot navigation or SLAM, but are familiar with \textbf{vibration measurements}, could information or data related to \textbf{vehicle dynamic conditions}, \textbf{time synchronization errors, and estimated position error be provided? }

This would help to determine what applications could be considered and time synchronization requirements.


****************************************

Reviewer 2 Comments

****************************************

\textcolor{green}{DONE} \mf{elaborate abstract, principle, implementation} The Abstract lacks important information regarding the proposed solution. No explanation on the working principle or how it was implemented has been given.

****************************************

Reviewer 3 Comments

****************************************

%This paper claims advantages of a sync system in precision and demonstrated comparison data results. 

\textcolor{green}{DONE} \mf{more technical details on system design} I suggest that it should include more explanations on the  design system of the hardware, software, and firmware.

****************************************

Reviewer 4 Comments

****************************************

\mf{expand results and methodology} 1. Significantly expand on the actual results and methodologies employed.

\textcolor{green}{DONE} \mf{technical description} 2. General lacks detail around the actual method employed.

========================================

IEEE SENSORS 2021 Conference

****************************************

Reviewer 1 Comments

****************************************

%This paper reports a new method for sensor synchronization using MCU. 

\mf{provide accuracy} But the reviewer did not find a clear timing accuracy to GNSS timed sensors.

****************************************

Reviewer 2 Comments

****************************************

%this paper presents a hardware synchronization solution for IMU Lidar. And their solution could achieve 1us level latency. As the internal timer of Lidar is microsecond level, such synchronization solution is eough for Lidar usages.
 
\mf{sync to error} In this paper, the Lidar+IMU robot is built for SLAM application, how time synchronization would help SLAM result?

is 10us or 100us enough to achieve low translation and rotation error?

\textcolor{green}{NONSENSE} \mf{impact of imu sampling to lidar sync} assume Velodyne LiDAR's sampling rate is 10Hz, IMU sampling rate is 1000Hz. Will high frequent IMU data transmission affects MCU timing?

\mf{citations must be cleaned up}

\mf{precision is predictable}

==> _reviews.tex <==
Dear Marsel Faizullin,

Thank you for submitting to the 2022 IEEE International Symposium on Inertial Sensors and Systems. We regret to inform you that your submission ID 2016 entitled "Open-Source Lidar Time Synchronization System by Mimicking GPS-Clock" was not selected for presentation at this year's conference. Please inform any coauthors of this decision.

Your submission was reviewed by the Technical Program Committee for technical merit, technical clarity and details, suitability for the overall conference program, and overlap with other submissions.  This year we had a large number of submissions and were forced to decline many fine contributions.

We appreciate your interest in the INERTIAL 2022 conference and invite you to participate in our conference from March 28-31 and enjoy the technical and social interaction with your colleagues. We encourage you to submit to our future conferences.

Sincerely,
The INERTIAL 2022 Organizing Committee


****************************************

Reviewer 1 Comments

****************************************

First off, the reviewer commends the authors efforts to create open-source software and detailed documentation of the needed hardware so that others may benefit from their work. However, in order to be suitable for acceptance, the reviewer notes that the following areas should be addressed:

-While the abstract format precludes providing exhaustive details of the method used for time synchronization, no details about how hardware time synchronization works is provided. 

The authors do note that this information will be released once accepted, but this introduces issues related to assessing the novelty of the work and potential limitations, for example, due to the underlying model or assumptions used for time synchronization. 

In regards to novelty, the authors third reference on Versavis is also on an open-source hardware time synchronization method that integrates with ROS. 

The authors need to clarify what is new or innovative. 

During initialization, Versavis triggers using a slow 1 Hz signal. 

This is very similar to a 1 PPS signal derived from GPS. 

In regards to modeling and assumptions, this information needs to be provided so that potential users can assess if the presented method is suitable for their application. 

For example, does this approach allow for sensors to be triggered and sampled independently or does the hardware enforce uniform triggering and sampling?

-The authors report an impressive time synchronization precision. 

However, given that sampling offsets between the IMU and LIDAR can introduce issues with SLAM, shouldn’t accuracy of time synchronization should also be assessed? 

If the authors can show that accuracy is not significant for their selected application of SLAM and that a biased but very precise time synchronization can be used, this would be an important result.

However, if accuracy is more important, this information should be reported.

-The authors note that time synchronization errors become a more significant issue during high dynamic conditions. 

To provide context to conference attendees that are not familiar with robot navigation or SLAM, but are familiar with vibration measurements, could information or data related to vehicle dynamic conditions, time synchronization errors, and estimated position error be provided? 

This would help to determine what applications could be considered and time synchronization requirements.


****************************************

Reviewer 2 Comments

****************************************

The Abstract lacks important information regarding the proposed solution. No explanation on the working principle or how it was implemented has been given.

****************************************

Reviewer 3 Comments

****************************************

This paper claims advantages of a sync system in precision and demonstrated comparison data results. 

I suggest that it should include more explanations on the  design system of the hardware, software, and firmware.


****************************************

Reviewer 4 Comments

****************************************

1. Significantly expand on the actual results and methodologies employed.

2. General lacks detail around the actual method employed.



========================================



Dear Marsel Faizullin,

Thank you for your submission to the IEEE SENSORS 2021 Conference. We regret to inform you that your submission number 1313 entitled "Open-Source Lidar Time Synchronization System by Mimicking GPS-Clock" was not selected for presentation at this year's Conference. Please inform any coauthors of this decision.

Your submission was reviewed by the Technical Program Committee for technical merit, suitability for the overall conference program, and overlap with other submissions.  This year we had a large number of submissions and were forced to decline many fine contributions. The reviewers' comments are included below for your information. The Technical Program Committee cannot give any further clarification and you do not need to explicitly respond to them.

We appreciate your interest in the IEEE SENSORS 2021 Conference and encourage you to attend the conference from October 31 - November 4, and enjoy the technical and social interaction with your colleagues.

Sincerely,
Technical Program Committee
IEEE SENSORS 2021 Conference




****************************************

Reviewer 1 Comments

****************************************

This paper reports a new method for sensor synchronization using MCU. 

But the reviewer did not find a clear timing accuracy to GPS timed sensors.

****************************************

Reviewer 2 Comments

****************************************

this paper presents a hardware synchronization solution for IMU Lidar. And their solution could achieve 1us level latency. As the internal timer of Lidar is microsecond level, such synchronization solution is eough for Lidar usages.
 
In this paper, the Lidar+IMU robot is built for SLAM application, how time synchronization would help SLAM result?

is 10us or 100us enough to achieve low translation and rotation error?

assume Velodyne LiDAR's sampling rate is 10Hz, IMU sampling rate is 1000Hz. Will high frequent IMU data transmission affects MCU timing?

==> trash/trash_.tex <==

The system has multi-modal sensors rigidly attached to a metal rig.

These sensors are Azure Kinect DK, Velodyne VLP-16 Lidar, Samsung S10e smartphone cameras and IMU-sensor. STM32F4DISCOVERY development board based on STM32F407 MCU and equipped by MPU9150 IMU-sensor. In addition Dell Latitude 5491 laptop is used for controlling synchronized data recording and post-processing.

Azure Kinect DK consist of a depth-camera. Other sensors including an RGB-camera, microphone array and IMU-sensor are not used in our work. We will refer to this sensor as depth-camera.

%gray-scale?
%Azure Kinect sensor has depth + gray-scale global shutter camera, RGB rolling shutter camera, imu, microphone array. We use only d+g camera. It supports external sync of cameras that we use for our system. 5 Hz.

%Lidar VLP-16 is used. Nothing to add. sync data from mcu. gps emulation with pps

The laptop is powered by Ubuntu 18.04 OS, Intel(R) Core(TM) i7-8850H CPU @ 2.60GHz, 16 GB DDR4 RAM. %, usb, ethernet, wifi, ...
Smartphone is powered by Android 10 OS,
\mf{for Azat} Samsung Exynos 9820 CPU @ 2.7GHz, dual camera, gyroscope, accelerometer, proximity and compass sensors. 
STM32F4DISCOVERY board is used for HW synchronization and imu data acquisition. We will call this as MCU board. These data is used primarily for software-based clock synchronization of smartphone data with the other sensors data.

Every sensor is connected to the laptop during recording. Depth-camera and board connected to the laptop through USB interface, lidar is connected by ethernet cable while smartphone shares common Wi-Fi access point. Smartphone also can work as access point.

%Every sensor apart from smartphone stores data on laptop and connected through usb and ethernet. Smartphone send some data only for sync purpose through Wifi. 

Since some of the sensors are well-known for robotics society we will only deeply describe MCU board. We will also consider smartphone usage in our system.

\subsection{Mcu imu board and firmware}

As mentioned above MCU board performs tasks for heterogeneous clock synchronization of the sensors.
The synchronisation tool is based on hardware triggering and interrupt handling to reach the highest possible accuracy (precision?) on MCU while preserving flexibility of programming and extending existing code. 

The board (i) handles depth camera triggering for one-time depth-images frame alignment with smartphone RGB-images
(ii) feeds lidar by required timestamps along with providing precise PPS pulses, (iii) gather timestamped IMU-data for further software-based clock synchronization algorithm~\cite{faizullin2021twist}, (iv) captures timestamps of triggered depth-camera frames for its further re-timestamping.

%tight design with hard sync, imu data, STM32 board, hw timers, hw rtc


%Below we will briefly describe every task.

%In addition it is equipped by signal UART interface signal inverter because Lidar has inverted signal diagram. CPU 76.8 MHz that were chosen as multiple of 19.2 Mhz - imu reference clock.

%Imu connected to via i2c and has additional 2 lines: (i) clock from mcu and interrupt signal from imu. Clock signal is needed because internal rc generator deviates and we need common clock source where we can get it. Interrupt signals are needed to be informed when to read data.

%mcu provides reference PPS for lidar and feed it by NMEA messages timestamps. By this it emulates gps receiver. + inverter for lidar

%mcu provides triggering pulses for depth camera. This is an actuatior to align depth data and smartphone rgb images by our Twist-n-Sync method.

%Since mcu is not fully temporally defined we decided just to check delays by oscilloscope. We have this delay... that is negligable.

\subsection{Smartphone sensors}
\mf{for Azat}
% app
% - Basic app workflow for sensor recording(?)
% - Synchronization of sensors with camera frames
To record smartphone sensor data, we use OpenCamera Sensors, \mf{underline that it is ours and the best thing you can imagine} ---  an Android application for synchronized recording of video and IMU data, 
%which is publicly available on GitHub. It records sensor data and video with frame timestamps synced to the same clock.
which is developed and maintained by our laboratory and is publicly available on GitHub. It records sensor data and video with frame timestamps synced to the same clock. 

% TODO: basic workflow

% - Special characteristics of the recording process 
%  - Constant frame rate
%  - Disable stabilization
%  - No sound recording
The recording process has the following specific properties, which are needed to minimize smartphone post-processing effects.
\begin{enumerate}
    \item As all the elements in the system have to be rigidly connected, we disable video stabilization. 
    \item Turning off sound recording is necessary to avoid the addition of extra frames by Camera2API software. 
    \item We lock exposure to achieve a constant frame rate, as autoexposure can produce "leaps" in frames when exposure changes.
\end{enumerate}

% - Limitations
%  - Camera2API support
%  - Synchronized timestamps feature support is required
OpenCamera Sensors has some software and hardware limitations. Firstly, the application requires Camera2API support for manipulations with camera frames. Another requirement is support for camera frame timestamps synchronization with the smartphone's internal clock, which is used for sensor timestamps.

\section{Software}



ROS. common api for the whole system. It is convenient way to build homogeneous software system with standard types of messages and standard ways to store and process them. It wrappes specific api of different vendors.

We returned original azure timestamps to get hw azure clock data. azure ros patched. Now Azure ros gives its internal ts that is more precisely align with mcu ts.

velodyne ros patched \mf{for Anastasiia} \ak{I'm not sure that there should be something specific -- we just need to say that we use GPS timestamps for LiDAR timestamp domain, less text - more schemes :) }.

Our own ros mcu
transform mcu data to ros imu and time ref messages and publish them for further purposes. This is also media for commands from master that control mcu. 

get imu data, setup azure trigger, publ sm to mcu offset

mcu firmaware 

imu data, triggering scheme, hw sync

Master. 

Connection with sm, mcu align control. Twistnsync, send messages to mcu


Sm-Laptop Communication \mf{for Azat}
% - Remote rec feature
% - Communication protocol
%   - Smartphone part, server part
We utilize OpenCamera Sensors remote control over the network feature to (a) load sensor recordings from the smartphone, (b) start and stop video recording, (c) obtain information about the frame timestamps phase during recording. The remote control feature consists of two main parts: the application, accepting requests according to the API, and the API client Python class, allowing one to send the requests and receive responses. The basic workflow for remote recording is to (1) connect PC and smartphone to the same network, (2) use API methods in Python code to control the application.

% Figure with available remote requests(?)

\section{Data gathering and Heterogeneous synchronization}

As mentioned above~\ref{} none of the sensors has analogous physical interface; because of that heterogeneous approach of synchronization is needed. 

We will describe these ways in this (sub)section.

We decided to utilise MCU clock as reference clock for every sensor. %Why? Why high-freq?


Since the most tightly connected sensor to and completely configured by IMU is IMU, we start with it. IMU has three physical interfaces for working with MCU. They are (i) I2C interface for data and commands transferring between MCU and IMU; (ii) interrupt signal driven by IMU that indicate IMU data ready event; (iii) highly accurate and stable reference clock signal generated by MCU to drive IMU. The reference clock is needed, firstly, to avoid use of IMU internal imprecise RC-generator~\cite{} and, secondly, to get synchronous work of MCU-IMU pair. The latter requirement allows one to have constant and predictable IMU frame period within MCU clock domain. This constrain is crucial for some algorithms utilizing inertial data, for instance preintegration technique in Visual-Inertial Odometry problem need IMU frame rate to be a multiple of visual camera frame rate~\cite{}. 

The next sensor. Lidar. Lidar cannot be configured by MCU but have hardware interface for connecting GPS-receiver for global time synchronization. The scheme receives ASCII messages by serial interface (HOW to call it?) and PPS (intro somewhere) pulses~\cite{}. We accommodate this feature for our hardware synchronization technique: by the MCU board we emulate GPS-receiver repeating the interface above. In addition there signal inverter needed to match MCU and Lidar physical layers on serial interface.

[Rewrite] Azure DK is designed with ability to use an external hardware trigger for exposure, this is usually used in applications with multiple depth-cameras where one of them generates trigger pulses and the others are treated as receivers of the signal. We utilize this feature and provide highly accurate trigger pulses by MCU board. (Only grid of some frame rates is permitted.) In this case we can trigger camera in exact time instances of MCU domain but we cannot provide these timestamps straightforward to the camera sensor. We have timestamps from MCU and Azure and we need matching. For that we monitor these two timestamp sequences. We have to solve problems in matching. We need 5 (or 15<30 fps) Azure support 5 Hz, but exposure randomly can start in k/30 sec because of internal logic. We decided to send trigger signals with 30 Hz, but set up Azure for 5 Hz fps. Than we match 12-th triggering pulse time and the second frame, this is because of the first Azure frame does not have correct time instance of 

Smartphone-to-MCU clock synchronization is fully software since no common information is available... 

1. Clock synchronization. Can be by NTP. But we choose Twist-n-Sync. Why? Doesn't depend on Net conditions. Smth else needed. 



2. Frame synchronization

based and uses timestamps of the first smartphone camera frame and computes offset that must be added to depth-camera triggering system. This offset is computed as 

\begin{align}
    dt = 
\end{align}


lightning OSCILL
\gf{more pictures from lights for alignments, calibration, some sequences, etc.}

We have several sensors and none of them has the same sync technique:

Lidar = latch + timestamps. This is full gps receiver emulation 

Azure = triggers

Imu = hw clocking + mcu i2c. Tightly coupled with mcu board

Sm = post-processing. Provides timestamps

\begin{table}[h]
\caption{An Example of a Table}
\label{table_emkfi}
\begin{center}
\begin{tabular}{l|l|l}
\textbf{Sensor} & \textbf{Sync method} & \textbf{Sync type}\\
\hline
Lidar & PPS + time messages & HW\\
Azure (D+G) & Triggering & HW\\
Imu & Clocking + Interrupts with mcu & HW\\
Sm camera & Clock alignment by \cite{faizullin2021twist} & SW\\
Sm imu & \textit{Clock alignment by \cite{faizullin2021twist}} & SW\\
\end{tabular}
\end{center}
\end{table}

\begin{table}[h]
\caption{An Example of a Table}
\label{table_example}
\begin{center}
\begin{tabular}{c|c|c|c|c|c|c}
\textbf{Sensor} & \multicolumn{2}{c|}{\textbf{Sync state after turn on}} & \multicolumn{2}{c|}{\textbf{Sync state align}} & \multicolumn{2}{c}{\textbf{Sync stt post-prc}}\\
\hline
& fr sync & clk sync & fr sync & clk sync & fr sync & clk sync\\
\hline
Lidar & \red & \green & \red & \green & \red & \green\\
\hline
Azure (D+G) & \red & \red & \red & \green & \green & \green\\
\hline
Imu & \red & \green & \red & \green & \red & \green\\
\hline
Sm camera & \red & \red & \red & \green & \green & \green \\
\hline
Sm imu
\end{tabular}
\end{center}
\end{table}


\subsection{Eval of Sm-to-Rest sync}

MCU CPU process comands and data in single thread. Here we are not about peripheral. So when we have interrupt signal of triggering pulse we measure timer counter to compute time. Number of CPU clocks between pulse and timer counter capture may vary because of possible handling interrupt with higher priority. Because of that we gather statistics on delay between pulse time instance and software pin response. Thus we can get higher bound of timestamping precision estimate.

For every sensor we have the following delays between hardware signal changes and time registration of these state switching.

$$\Delta_{pulse-response} = 3.47 \pm 0.0024\, \si{\micro\second}$$
$$\Delta_{pulse-response} = 1000000 \pm 700000$$
$$\Delta_{pulse-response} = 4000000 \pm 9000000$$

There is 3 us delay. In this paper we do not consider reasons of the delays, but it is related to high level api that we use for mcu firmware \cite{}. This has some overhead. In addition spend for interrupt handling. 


\section{Trajectory estimation}
\ak{Discussion on traj estimation results}

Since the developed setup provides smartphone data well-synchronized with external multi-modal high-precision sensors (depth camera, LiDAR), this gives an opportunity to calculate smartphone's trajectory in a wide range of environments. In our work we will divide them in two groups: (i) small-scale environments, that can be scanned in details via depth camera, and (ii) large-scale environments, that can be efficiently covered by long-range sensors like LiDAR.

We've considered the next concepts for estimation setup trajectory: monocular RGB for both (i) and (ii), RGB-D for (i), LiDAR for (ii). For every of the mentioned direction, we used the next state-of-the-art representatives with open-source implementation: COLMAP~\cite{schoenberger2016sfm} software for Structure-from-Motion for RGB data, ORB-SLAM2~\cite{murORB2} for RGBD data, and LOAM algorithm~\cite{zhang2014loam} for LiDAR data.




The main criteria for estimation algorithm quality were algorithm' performance and subjective quality assessment of the estimated trajectory. From the performance perspective of view, ORB-SLAM2 and LOAM produce real-time results, whereas COLMAP reqiures ??? \ak{don't know values}. \ak{Comment somehow quality of trajectories}.

\section{Conclusion}

\section{[must be added]}

no frame-scale cam to imu sync. We do not need this. can be added by our twist n sync

We do not need 30 Hz, so we use 5 only, but 30 Hz is trigger freq and you can o 30

delay dependent/independent on other interrupts?

measure delay between int and led on

measure delay between signal and led on

measure delay between trig and led on

mcu firm:
mcu soft:
master:

Clocking uncertainty. timestamps vs. reality

